XPC: Fast and Reliable Synchronous Transmission Protocols for 2-Phase Commit and 3-Phase Commit

One of the major challenges for the engineering of wireless sensing systems is to improve the software abstractions and frameworks that are available to programmers while ensuring system reliability and efficiency. The distributed systems community have developed a rich set of such abstractions for building dependable distributed systems connected using wired networks, however after 20 years research many of these elude wireless sensor systems. In this paper we present X Process Commit (XPC) an atomic commit protocol framework that utilizes Synchronous Transmission (ST). We also introduce Hybrid, a technique that allows us to exploit the advantages of the Glossy and Chaos Synchronous Transmission primitives to get lower latency and higher reliability than either. Using XPC and Hybrid we demonstrate how to build protocols for the classical 2-phase and 3-phase commit abstractions and evaluate these demonstrating significantly improved performance and reliability than the use of Glossy or Chaos individually as dissemination primitives. We address how we overcame the timing challenges of bringing Glossy and Chaos together to form Hybrid and through extensive experimentation demonstrate that it is robust to in-network radio interference caused by multiple sources. We are first to present testbed results that show that Hybrid can provide almost 100% reliability in a network of nodes suffering from various levels of radio interference.

==> Sections/OLD_Intro.tex <==
\section{Introduction}

Wireless Sensor Networks (WSN) are made of several small MEMS (Micro
Electro-Mechanical Systems) computers equipped with sensors, radio
transceivers, and batteries. These sensor nodes enable the creation of many novel sensing
applications due to their small size and ease of deployment. Common application
areas include precision agriculture \cite{baggio2005wireless} and the
monitoring of civil infrastructure such as bridges \cite{stajano2010smart}.
In many of these cases in-network processing is used
\cite{kolcun2016efficient}. 

The sensor nodes of a WSN need the ability to reach an agreement in a
distributed way on new data. This ability can be used to 
support system configuration like the choice of a new sample rate for sensing
applications \cite{baggio2005wireless}, \cite{stajano2010smart}, or for the
decision to update to a new software image \cite{langiuupkit}. 

%%% Voting protocols are...
This is a transaction agreement, an example of the distributed database commit problem
\cite{lynch1996distributed}. The goal is for all of the nodes in a system
to either accept an update, or reject the update. There are two accepted
protocols to achieve uniform commits, a two-phase commit (2PC), or a
three-phase commit (3PC). 

The problem is that both of these protocols require reliable communication from all of
the nodes of the network. This makes their use in WSN difficult
due to the unreliable nature of radio communication, and the high loss rate of
WSN sensor nodes \cite{breza2018failures}.

%%% 2PC is ....

%%% 3PC is ...

%Paxos \cite{paxos} is a widely used consensus protocol which
%ensures protocol safety and liveliness using majority-based
%network-wide voting. Paxos requires a large amount of reliable communication.
%This requirement poses two problems. The first is that WSN sensor nodes have a
%limited amount of energy because they are powered by batteries, or are
%harvesting energy from the environment at an unpredictable rate. One of the
%largest consumers of energy for a WSN sensor node is radio communication. The
%other problem is that low-powered radio communication is unreliable. These are
%both challenges to the use of Paxos on WSN.
%
%Wireless Paxos \cite{wpaxos} (WP) is a Paxos consensus protocol for WSN. It
%uses the Chaos \cite{chaos} all-to-all communication primitive based on Synchronous
%Transmissions (ST) \cite{baloo}. WP successfully provides consensus for WSN
%sensor nodes, but suffers from network instability and can fail to terminate in
%some cases.

Synchronous Transmission (ST) \cite{baloo} is a wireless communication
approach where nodes are tightly synchronised and communicate at the same time. 
If the messages are the exact same and arrive at a receiver within $0.5
\mu$seconds then the messages will constructively interfere, and be received
correctly. If the messages are different, and arrive within $160\mu$seconds and
have a $3Db$ difference in signal strength, then the stronger signal will be
successfully received in spite of the presence of another signal. This is
called non-destructive interference.

Glossy is a reliable, one-to-all ST communication primitive \cite{glossy}. 
It has been experimentally shown to provide reliable
communication even in the presence of network interference. As Glossy is
one-to-all, it can only handle communication serially.

Chaos \cite{chaos} is an all-to-all ST communication primitive used to
disseminate information to WSN sensor nodes. As an all-to-all primitive it can
terminate much faster than Glossy, but, its performance can suffer from
network instability and it can fail to terminate in some cases.

In this paper we present XPC, a voting library to support transactional
protocols that utilises Synchronous Transmissions. XPC uses ST 
because the protocols need reliable communication links to work. We use our
library to assess two commonly used ST approaches, Glossy and Chaos, and
propose the use of a third hybrid approach, made possible by XPC, that combines
the best aspects of both of the primitives. We evaluate the latency and
reliability of XPC and the hybrid ST approach on a WSN testbed.

%In this paper we do an analysis of the reliability and performance of these two
%different ST approaches when applied to voting protocols. We then present our
%own hybrid ST primitive that tries to get the best of both approaches for the
%purposes of fast and reliable communication for voting protocols.

Contributions:
\begin{itemize}

\item We present a library 
to reliably implement voting protocols on WSN sensor nodes using Synchronous
Transmission.

\item We evaluate different Synchronous Transmission primitive to see their
performance and reliability under various network conditions.

\item We present an approach to combine Glossy and Chaos into a fast and
reliable communication primitive to support WSN protocols.  
%This is a contribution in
%its own right because the control communication for each is different.

\end{itemize}



==> Sections/Related_Work.tex <==
\section{Related\_Work}


==> evaluation/flocklab-interference.tex <==
\begin{table}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccc|} \toprule
    %% LOW INTERFERENCE %%
    {\textbf{Low Interference}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
     \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{100.00} & \multirow{2}{*}{222.95} & \textbf{P1}: 98.51 & \textbf{P1}: 1.10 \\
            & & & \textbf{P2}: 99.27 & \textbf{P2}: 1.07 \\ \midrule
     \multirow{3}{*}{3PC-Hybrid} & \multirow{3}{*}{100.00} & \multirow{3}{*}{333.72} & \textbf{P1}: 98.74 & \textbf{P1}: 1.11 \\
            & & & \textbf{P2}: 98.99 & \textbf{P2}: 1.12 \\
            & & & \textbf{P3}: 99.63 & \textbf{P3}: 1.01 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{215.87} & \textbf{MP}: 98.49 & \textbf{MP}: 1.00 \\
            & & & \textbf{DP}: 99.46 & \textbf{DP}: 1.09 \\ \midrule
    \multirow{2}{*}{WIMP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{329.25} & \textbf{MP}: 98.58 & \textbf{MP}: 1.00 \\
            & & & \textbf{DP}: 98.47 & \textbf{DP}: 1.15 \\ \midrule
    %% HIGH INTERFERENCE %%
    {\textbf{High Interference}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
    \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{100.00} & \multirow{2}{*}{304.19} & \textbf{P1}: 92.83 & \textbf{P1}: 1.52 \\
            & & & \textbf{P2}: 88.38 & \textbf{P2}: 1.59 \\ \midrule
     \multirow{3}{*}{3PC-Hybrid} & \multirow{3}{*}{100.00} & \multirow{3}{*}{432.14} & \textbf{P1}: 94.81 & \textbf{P1}: 1.40 \\
            & & & \textbf{P2}: 94.38 & \textbf{P2}: 1.52 \\
            & & & \textbf{P3}: 94.39 & \textbf{P3}: 1.51 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{241.43} & \textbf{MP}: 93.40 & \textbf{MP}: 1.01 \\
            & & & \textbf{DP}: 97.41 & \textbf{DP}: 1.47 \\ \midrule
    \multirow{2}{*}{WIMP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{350.25} & \textbf{MP}: 93.61 & \textbf{MP}: 1.00 \\
            & & & \textbf{DP}: 92.57 & \textbf{DP}: 1.54 \\ \midrule
    %% WIFI INTERFERENCE %%
    {\textbf{Wifi Interference}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
    \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{100.00} & \multirow{2}{*}{383.07} & \textbf{P1}: 92.19 & \textbf{P1}: 2.29 \\
            & & & \textbf{P2}: 90.54 & \textbf{P2}: 2.19 \\ \midrule
     \multirow{3}{*}{3PC-Hybrid} & \multirow{3}{*}{100.00} & \multirow{3}{*}{606.20} & \textbf{P1}: 91.32 & \textbf{P1}: 2.26 \\
            & & & \textbf{P2}: 92.92 & \textbf{P2}: 1.96 \\
            & & & \textbf{P3}: 89.58 & \textbf{P3}: 2.31 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{270.93} & \textbf{MP}: 87.79 & \textbf{MP}: 1.05 \\
            & & & \textbf{DP}: 91.98 & \textbf{DP}: 1.44 \\ \midrule
    \multirow{2}{*}{WIMP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{360.88} & \textbf{MP}: 86.09 & \textbf{MP}: 1.04 \\
            & & & \textbf{DP}: 91.98 & \textbf{DP}: 1.70 \\ \midrule
    %% MICRO INTERFERENCE %%
    {\textbf{Microwave}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
    \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{100.00} & \multirow{2}{*}{396.06} & \textbf{P1}: 92.97 & \textbf{P1}: 2.07 \\
            & & & \textbf{P2}: 91.82 & \textbf{P2}: 2.17 \\ \midrule
     \multirow{3}{*}{3PC-Hybrid} & \multirow{3}{*}{100.00} & \multirow{3}{*}{586.67} & \textbf{P1}: 92.09 & \textbf{P1}: 1.95 \\
            & & & \textbf{P2}: 91.58 & \textbf{P2}: 2.12 \\
            & & & \textbf{P3}: 92.30 & \textbf{P3}: 1.95 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{342.53} & \textbf{MP}: 78.90 & \textbf{MP}: 1.15 \\
            & & & \textbf{DP}: 91.14 & \textbf{DP}: 2.23 \\ \midrule
    \multirow{2}{*}{WIMP} & \multirow{2}{*}{100.00} & \multirow{2}{*}{377.31} & \textbf{MP}: 86.22 & \textbf{MP}: 1.01 \\
            & & & \textbf{DP}: 91.69 & \textbf{DP}: 1.66 \\ \midrule
\end{tabular}}
\end{center}

\caption{Comparison of XPC protocol implementations across varying interference levels.} \label{table:evaluation-global}
\end{table}


==> evaluation/flocklab-multiference.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccc|} \toprule
    %% MICROWAVE 2 NODES %%
    {\textbf{Microwave (2 Nodes)}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
     \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{100.00} & \multirow{2}{*}{1027.18} & \textbf{P1}: 82.91 & \textbf{P1}: 4.64 \\
            & & & \textbf{P2}: 81.54 & \textbf{P2}: 5.04 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{98.33} & \multirow{2}{*}{625.37} & \textbf{MP}: 56.49 & \textbf{MP}: 1.57 \\
            & & & \textbf{DP}: 82.85 & \textbf{DP}: 4.52 \\ \midrule
    %% MICROWAVE 3 NODES %%
    {\textbf{Microwave (3 Nodes)}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
     \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{95.92} & \multirow{2}{*}{1025.86} & \textbf{P1}: 80.26 & \textbf{P1}: 4.95 \\
            & & & \textbf{P2}: 81.43 & \textbf{P2}: 5.11 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{92.86} & \multirow{2}{*}{756.73} & \textbf{MP}: 47.00 & \textbf{MP}: 1.97 \\
            & & & \textbf{DP}: 81.37 & \textbf{DP}: 5.22 \\ \midrule
    %% MICROWAVE 4 NODES %%
    {\textbf{Microwave (4 Nodes)}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
     \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{57.14} & \multirow{2}{*}{1221.30} & \textbf{P1}: 79.59 & \textbf{P1}: 6.72 \\
            & & & \textbf{P2}: 79.92 & \textbf{P2}: 6.11 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{59.18} & \multirow{2}{*}{1024.20} & \textbf{MP}: 42.06 & \textbf{MP}: 2.27 \\
            & & & \textbf{DP}: 78.83 & \textbf{DP}: 6.91 \\ \midrule
    %% MICROWAVE 5 NODES %%
    {\textbf{Microwave (5 Nodes)}} & {\textbf{Reliability (\%)}} & {\textbf{Latency (ms)}} & {\textbf{Chaos Coverage (\%)}}& {\textbf{Avg. Retr.}}  \\ \midrule
     \multirow{2}{*}{2PC-Hybrid} & \multirow{2}{*}{47.22} & \multirow{2}{*}{1291.68} & \textbf{P1}: 75.51 & \textbf{P1}: 7.85 \\
            & & & \textbf{P2}: 79.37 & \textbf{P2}: 7.50 \\ \midrule
    \multirow{2}{*}{WISP} & \multirow{2}{*}{59.09} & \multirow{2}{*}{1178.84} & \textbf{MP}: 41.67 & \textbf{MP}: 2.83 \\
            & & & \textbf{DP}: 73.88 & \textbf{DP}: 7.67 \\ \midrule
\end{tabular}}
\end{center}

\caption{2PC and WISP analysis with increasing levels of JamLab microwave interference.} \label{table:evaluation-multiference}
\end{table}

